Learning Factorized Multimodal Representations

Learning multimodal representations is a fundamentally complex research problem due to the presence of multiple heterogeneous sources of information. Although the presence of multiple modalities provides additional valuable information, there are two key challenges to address when learning from multimodal data: 1) models must learn the complex intra-modal and cross-modal interactions for prediction and 2) models must be robust to unexpected missing or noisy modalities during testing. In this paper, we propose to optimize for a joint generative-discriminative objective across multimodal data and labels. We introduce a model that factorizes representations into two sets of independent factors: multimodal discriminative and modality-specific generative factors. Multimodal discriminative factors are shared across all modalities and contain joint multimodal features required for discriminative tasks such as sentiment prediction. Modality-specific generative factors are unique for each modality and contain the information required for generating data. Experimental results show that our model is able to learn meaningful multimodal representations that achieve state-of-the-art or competitive performance on six multimodal datasets. Our model demonstrates flexible generative capabilities by conditioning on independent factors and can reconstruct missing modalities without significantly impacting performance. Lastly, we interpret our factorized representations to understand the interactions that influence multimodal learning.

==> figs_tex/ab_interp.tex <==

\begin{figure}[t!]
    \centering
    \begin{minipage}{0.37\textwidth}
        \centering
        \captionsetup{labelformat=empty}
        \caption{\small Table 2: Results for ablation studies on CMU-MOSI. Best results in bold.
}
\fontsize{7}{9}\selectfont
%\centering
\setlength\tabcolsep{0.9pt}

\begin{tabular}{|c || *{5}{K{0.9cm}} |}
\hline
Dataset & \multicolumn{5}{|c|}{\textbf{CMU-MOSI}}\\
Task & \multicolumn{5}{c|}{Sentiment} \\
Metric  & MAE & Corr  & A$^{2}$ & F1 & A$^{7}$\\ 
\hline \hline
$\mathbf{M}_\mathbf{E}$  & 1.043 & 0.634 & 76.1 & 76.0 & 28.7 \\
$\mathbf{M}_\mathbf{D}$  & 1.024 & 0.626 & 74.6 & 74.7 & 28.7 \\
$\mathbf{M}_\mathbf{C}$  & 1.071 & 0.647 & 76.5 & 76.5 & 31.9 \\
$\mathbf{M}_\mathbf{B}$  & 1.023 & 0.627 & 74.9 & 75.0 & 33.1 \\
$\mathbf{M}_\mathbf{A}$  & 1.039 & 0.645 & 75.1 & 75.1 & 32.4 \\
\ours  & \textbf{0.961} & \textbf{0.661} & \textbf{77.3} & \textbf{77.2} & \textbf{35.4} \\
\hline
\end{tabular}
\fontsize{7}{9}\selectfont
	\centering
\vspace{1mm}
\captionsetup{labelformat=empty}
        \caption{\small Table 3: Results for ablation studies on CMU-MOSI. Best results in bold.
\vspace{-2mm}}
    \begin{tabular}{| c || *{3}{K{1.3cm}}|}
\hline
Metric		& $r_\ell$ & $r_v$ & $r_a$ \\ 
\hline \hline
CMU-MOSI	& 0.3066 & 0.0301 & 0.1072 \\
POM		& 1.090 & 0.996 & 0.898 \\
\hline
\end{tabular}
    \end{minipage}%
    \begin{minipage}{0.6\textwidth}
        \centering
       \includegraphics[width=\linewidth]{./fig/local2.pdf}
        \captionsetup{labelformat=empty}
    \caption{(b)\vspace{1mm}}
	\caption{\small Local interpretations of multimodal representations on CMU-MOSI. We plot $\triangledown_{f_{y}} (\hat{x}_i)$ over time to assess the influence of $f_y$ on a sequence $\hat{x}_i$. $i \in \{ (\ell)anguage, (v)isual, (a)coustic \} $. Multimodal communicative behaviors that are strongly indicative of speaker sentiment such as positive words and informative acoustic features indeed correspond to increases in $\triangledown_{f_{y}} (\hat{x}_i)$. Behaviors ``very profound and deep'' in the language modality, slight smile in the visual modality as well as hesitant and emphasized tone of voice in the acoustic modality are highlighted.\vspace{-4mm}}
    \end{minipage}
\end{figure}

==> figs_tex/ab_new.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\definecolor{gg}{RGB}{45,190,45}

\begin{table}[t!]
\vspace{2mm}
\caption{\small Results for ablation studies on CMU-MOSI. Best results in bold. All the components in \ours \ are necessary for best performance.
}
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{1.2pt}
\centering
\begin{tabular}{|c||*{3}{K{1.5cm}:}*{1}{K{1.5cm}|}|*{5}{K{0.8cm}}||*{2}{K{0.8cm}}|}
\hline
\multirow{3}{*}{Variants} & Multimodal   & Hybrid      & Factorized  & Modal.-Speci.   & \multicolumn{5}{c||}{CMU-MOSI} & \multicolumn{2}{c|}{ICT-MMMO} \\
                          & Discriminative & Gen.-Discr. & Gen.-Discr. & Generative & \multicolumn{5}{c||}{Sentiment}  & \multicolumn{2}{c|}{Sentiment}                                           \\
                          & Factor     & Objective   & Factors     & Factors  & Acc(2) & F1  & Acc(7) & MAE & $r$ & Acc(2) & F1         \\ \hline \hline
$\mathbf{M_D}$                        & no         & no          & --          & --   & 75.2   & 75.2 & 33.2  & 1.020  & 0.616  & - & -   \\
$\mathbf{M_E}$                        & yes        & no          & --          & --            & 77.4         & 77.3          & 34.1         & 0.965          & 0.632    & - & -     \\
$\mathbf{M_B}$                       & no         & yes         & no          & --            & 75.9   & 76.0  & 34.8 & 0.979  & 0.640  & - & - \\
$\mathbf{M_C}$                       & yes        & yes         & no          & --            & 77.4          & 77.2          & 35.0    & 0.960  & 0.649 & - & - \\
$\mathbf{M_A}$                       & yes        & yes         & yes         & no            & 77.1 & 76.6 & 34.0          & 0.957 & 0.654 & - & - \\
$\mathbf{MFM}$                      & yes        & yes         & yes         & yes           & \textbf{78.1} & \textbf{78.1} & \textbf{36.2} & \textbf{0.963} & \textbf{0.662} & - & - \\ \hline
\end{tabular}
\vspace{-1mm}
\label{ab}
\end{table}

==> figs_tex/control.tex <==
\iffalse
\begin{figure*}[t!]
	\centering
	\includegraphics[width=1.0\textwidth]{./fig/control_z_new.pdf}
	%\vspace{-5mm}
	\caption{\small Image generation for SVHN \citep{noauthororeditor} and MNIST \citep{Lecun98gradient-basedlearning} digits. $\mathbf{Z_a}_{1}$, $\mathbf{Z_a}_{2}$, and $\mathbf{Z_y}$ refer to the {\em SVHN-specific generative}, {\em MNIST-specific generative}, and {\em multimodal discriminative} latent variables.
    }
	\label{fig:control}
\end{figure*}
\fi

==> figs_tex/interp.tex <==
%\begin{center}
\begin{figure}[t!]
    %\centering
    \begin{minipage}{0.4\textwidth}
        \fontsize{7.5}{10}\selectfont
        \setlength\tabcolsep{1.3pt}
        \begin{tabular}{l : *{6}{K{1.3cm}}}
        \Xhline{3\arrayrulewidth}
        Metric & $r_{\ell}$ & $r_v$ & $r_a$ \\
        \Xhline{0.5\arrayrulewidth} 
        CMU-MOSI& 0.3066 & 0.0301 & 0.1072 \\
        POM		& 1.090 & 0.996 & 0.898 \\
        POM		& 1.090 & 0.996 & 0.898 \\
        POM		& 1.090 & 0.996 & 0.898 \\
        POM		& 1.090 & 0.996 & 0.898 \\
        POM		& 1.090 & 0.996 & 0.898 \\
        \Xhline{3\arrayrulewidth}
        \end{tabular}
        \captionsetup{labelformat=empty}
        \caption{(b)\color{red} not yet finished.....}
        \label{global}
    \end{minipage}
    \begin{minipage}{0.6\textwidth}
        %\centering
        %\hspace{-4mm} 
    \includegraphics[width=\linewidth]{fig/local2.pdf}
        \captionsetup{labelformat=empty}
        \caption{(a)\vspace{2mm}}
    \end{minipage}
\caption{\small (a) Global interpretation results showing ratios $r_i = \frac{\textrm{Depen}(\mathbf{F_y},\hat{\mathbf{X}}_{i})}{\textrm{Depen}(\mathbf{F_a}_{i},\hat{\mathbf{X}}_{i})}$, $i \in \{ (\ell)anguage, (v)isual, (a)coustic \} $. The language and acoustic modalities contribute most to sentiment prediction. (b) Local interpretations of multimodal representations on CMU-MOSI by plotting $\triangledown_{f_{y}} (\hat{x}_i)$ over time to assess the influence of $f_y$ on a sequence $\hat{x}_i$. $i \in \{ (\ell)anguage, (v)isual, (a)coustic \} $. Multimodal communicative behaviors that are strongly correlated with displays of sentiment are highlighted by increases in $\triangledown_{f_{y}} (\hat{x}_i)$. Behaviors ``very profound and deep'' in the language modality, slight smile in the visual modality as well as hesitant and emphasized tone of voice in the acoustic modality are highlighted.\vspace{-4mm}}
\label{fig:interp}
\end{figure}
%\end{center}

==> figs_tex/local.tex <==
\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{./fig/local.pdf}
	%\vspace{-5mm}
	\caption{\small Local interpretations of multimodal representations on CMU-MOSI. We plot $\triangledown_{f_{y}} (\hat{x}_i)$ over time to assess the influence of $f_y$ on a sequence $\hat{x}_i$. $i \in \{ (\ell)anguage, (v)isual, (a)coustic \} $. Multimodal communicative behaviors that are strongly indicative of speaker sentiment such as positive words and informative acoustic features indeed correspond to increases in $\triangledown_{f_{y}} (\hat{x}_i)$. Behaviors ``very profound and deep'' in the language modality, slight smile in the visual modality as well as hesitant and emphasized tone of voice in the acoustic modality are highlighted.\vspace{-8mm}}
	\label{fig:local}
\end{figure*}

==> sections/SVHN_MNIST.tex <==
\section{Experiments}
\label{sec:exp}

\subsection{Multimodal Static Data}
\input{figs_tex/control_v2.tex}

In this section, we study an example that considers SVHN \citep{noauthororeditor} and MNIST \citep{Lecun98gradient-basedlearning} as two modalities. SVHN and MNIST are digit images with different styles but same labels (digits $0\sim 9$). We randomly pair $100,000$ SVHN and MNIST images with the same label. $80,000$ pairs are used for training and the rest are for testing. To justify that \ours \ is able to learn {\em multimodal discriminative} factors and {\em modality-specific generative} factors in multimodal data, we perform the classification task as well as the generation task in Figure \ref{fig:control}.

We perform experiments on both unimodal classification and multimodal classification tasks. For multimodal classification, we denote MM as a multimodal baseline that performs pure discriminative predictions given two modalities as inputs. We compare the results for unimodal classification, MM, and \ours \ in Figure \ref{fig:control} (b). This toy example explains that we can achieve better classification performance from unimodal to multimodal, and this is not surprising since more information are given. Moreover, the learned disentangled multimodal representations in \ours \ outperforms MM, which verifies the claim that we can use \ours \ to learn disentangled {\em discriminative} factors.

For the generation task, we denote the generative network of \ours \ in Figure \ref{fig:control} (a). Then, we generate the images with randomly sampled $\mathbf{Z_a}_1$, $\mathbf{Z_a}_2$, and $\mathbf{Z_y}$ from the prior. In Fig. \ref{fig:control} (c), \ours \ shows excellent capabilities in disentangling {\em multimodal discriminative} factors and {\em modality-specific generative} factors, allowing for flexible and accurate generation based on label or style.

In the next section, we move from multimodal static data to more challenging multimodal time-series data, where we study \ours \ in the intersection of language, visual and acoustic modalities.

==> tables/ab.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\definecolor{gg}{RGB}{45,190,45}

\begin{table}[h]
\vspace{-4mm}
\caption{\small Results for ablation studies on CMU-MOSI. Best results in bold. All the components in \ours \ are necessary for best performance.
}
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{1.2pt}
\centering
\vspace{-2mm}
\begin{tabular}{|c||*{3}{K{1.5cm}:}*{1}{K{1.5cm}|}|*{5}{K{0.8cm}}||*{2}{K{0.8cm}}|}
\hline
\multirow{3}{*}{Variants} & Multimodal   & Hybrid      & Factorized  & Modal.-Speci.   & \multicolumn{5}{c||}{CMU-MOSI} & \multicolumn{2}{c|}{ICT-MMMO} \\
                          & Discriminative & Gen.-Discr. & Gen.-Discr. & Generative & \multicolumn{5}{c||}{Sentiment}  & \multicolumn{2}{c|}{Sentiment}                                           \\
                          & Factor     & Objective   & Factors     & Factors  & Acc(2) & F1  & Acc(7) & MAE & $r$ & Acc(2) & F1         \\ \hline \hline
$\mathbf{M_E}$                        & no         & no          & --          & --   & 75.2   & 75.2 & 33.2  & 1.020  & 0.616  & - & -   \\
$\mathbf{M_D}$                        & yes        & no          & --          & --            & 77.4         & 77.3          & 34.1         & 0.965          & 0.632    & 73.8 & 73.1 \\
$\mathbf{M_C}$                       & no         & yes         & no          & --            & 75.9   & 76.0  & 34.8 & 0.979  & 0.640  & - & - \\
$\mathbf{M_B}$                       & yes        & yes         & no          & --            & 77.4          & 77.2          & 35.0    & 0.960  & 0.649 & - & - \\
$\mathbf{M_A}$                       & yes        & yes         & yes         & no            & 77.1 & 76.6 & 34.0          & 0.957 & 0.654 & - & - \\
$\mathbf{MFM}$                      & yes        & yes         & yes         & yes           & \textbf{78.1} & \textbf{78.1} & \textbf{36.2} & \textbf{0.963} & \textbf{0.662} & \textbf{81.3} & \textbf{79.2} \\ \hline
\end{tabular}
\vspace{-1mm}
\label{ab}
\end{table}

==> tables/ab_supple.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\definecolor{gg}{RGB}{45,190,45}

\begin{table}[t!]
\fontsize{7.5}{10}\selectfont
%\centering
\setlength\tabcolsep{1.1pt}
\begin{tabular}{l : *{5}{K{0.97cm}} : l : *{5}{K{0.97cm}}}
\Xhline{3\arrayrulewidth}
Dataset & \multicolumn{5}{c:}{\textbf{CMU-MOSI}} & Dataset & \multicolumn{5}{c}{\textbf{CMU-MOSI}} \\
Task & \multicolumn{5}{c:}{Sentiment} & Task & \multicolumn{5}{c}{Sentiment} \\
Metric  & A$^{2}$ & F1 & A$^{7}$ & MAE & Corr & Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & Corr \\ 
\Xhline{0.5\arrayrulewidth}
EF MM    & & & & & & MARN MM   & & & & &  \\
EF \ds    & 75.1 & 74.6 & 33.5 & 1.02 & \textbf{0.639} & MARN \ds  & 74.8 & 74.8 & 30.6 & 1.05 & 0.617 \\
EF \threes   & 74.9 & 75.0 & 33.1 & 1.02 & 0.627 & MARN \threes & 74.9 & 75.0 & \textbf{33.1} & \textbf{1.02} & 0.627 \\
EF GDDM    & & & & & & MARN GDDM   & & & & &  \\
EF \ones   & 74.8 & 74.7 & \textbf{33.7} & 1.03 & 0.627 & MARN \ones & 72.3 & 72.4 & 26.4 & 1.10 & 0.596 \\
EF \ours   & \textbf{75.2} & \textbf{75.3} & 32.8 & \textbf{1.02} & 0.629 & MARN \ours & \textbf{75.5} & \textbf{75.4} & 31.2 & 1.05 & \textbf{0.640} \\
\Xhline{0.5\arrayrulewidth}
TF MM    & & & & & & MFN MM   & 74.6 & 74.7 & 28.7 & 1.024 & 0.626 \\
TF \ds    & 75.1 & 75.1 & 27.0 & 1.10 & 0.643 & MFN \ds   & 76.1 & 76.0 & 28.7 & 1.043 & 0.634 \\
TF \threes   & 74.9 & 75.0 & \textbf{33.1} & \textbf{1.02} & 0.627 & MFN \threes & 74.9 & 75.0 & 33.1 & 1.023 & 0.627 \\
TF GDDM    & & & & & & MFN GDDM   & 74.3 & 74.4 & 31.9 & 1.039 & 0.610 \\
TF \ones   & 74.2 & 74.3 & 29.6 & 1.05 & 0.620 & MFN \ones  & 76.5 & 76.5 & 31.9 & 1.071 & 0.647 \\
TF \ours   & \textbf{75.5} & \textbf{75.4} & 30.9 & 1.05 & \textbf{0.648} & MFN \ours  & \textbf{77.3} & \textbf{77.2} & \textbf{35.4} & \textbf{0.961} & \textbf{0.661} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Sentiment prediction results on CMU-MOSI test set for comparing the performance of \ours \ with ablation baselines. Best scores per fusion model are indicated in bold. \ours \ generally achieves better results as compared to ablation baselines that remove disentangled and generative capabilities. A$^C$ = multiclass accuracy across $C$ classes, MAE = Mean Absolute Error, $r$ = Pearson's correlation.}
\label{ab_supple}
\end{table}

==> tables/global.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\definecolor{gg}{RGB}{45,190,45}

\begin{wraptable}{r}{6.0cm}
\fontsize{7.5}{10}\selectfont
%\centering
\setlength\tabcolsep{1.3pt}
\begin{tabular}{l : *{6}{K{1.3cm}}}
\Xhline{3\arrayrulewidth}
Metric		& $\frac{\textrm{MI}(\mathbf{F_y},\hat{\mathbf{X}}_{\ell})}{\textrm{MI}(\mathbf{F_a}_{\ell},\hat{\mathbf{X}}_{\ell})}$ & $\frac{\textrm{MI}(\mathbf{F_y},\hat{\mathbf{X}}_{v})}{\textrm{MI}(\mathbf{F_a}_{v},\hat{\mathbf{X}}_{v})}$ & $\frac{\textrm{MI}(\mathbf{F_y},\hat{\mathbf{X}}_{a})}{\textrm{MI}(\mathbf{F_a}_{a},\hat{\mathbf{X}}_{a})}$ \\ 
\Xhline{0.5\arrayrulewidth}
CMU-MOSI	& 0.3066 & 0.0301 & 0.1072 \\
POM		& 1.090 & 0.996 & 0.898 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Global interpretation on CMU-MOSI for multimodal sentiment analysis. $i \in \{ (\ell)anguage, (v)isual, (a)coustic \} $. The language and acoustic modalities contribute most to sentiment prediction.}
\label{global}
\end{wraptable}

==> tables/mmmo.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\definecolor{gg}{RGB}{45,190,45}

\begin{table}[tb]
\fontsize{7.5}{10}\selectfont
%\centering
\setlength\tabcolsep{1.0pt}
\begin{tabular}{l : *{2}{K{0.93cm}} : *{2}{K{0.93cm}} : *{2}{K{0.93cm}}}
\Xhline{3\arrayrulewidth}
Dataset & \multicolumn{2}{c:}{\textbf{ICT-MMMO}} & \multicolumn{2}{c:}{\textbf{YouTube}} & \multicolumn{2}{c}{\textbf{MOUD}} \\
Task & \multicolumn{2}{c:}{Sentiment} & \multicolumn{2}{c:}{Sentiment} & \multicolumn{2}{c}{Sentiment} \\
Metric       	& A$^{2}$ & F1 & A$^{3}$ & F1 & A$^{2}$ & F1 \\ 
\Xhline{0.5\arrayrulewidth}
Majority		& 40.0 & 22.9 & 42.4 & 25.2 & 60.4 & 45.5\\
RF				& 70.0 & 69.8 & 33.3 & 32.3 & 64.2 & 63.3\\
SVM     		& 68.8 & 68.7 & 42.4 & 37.9 & 59.4 & 45.5\\
THMM			& 53.8 & 53.0 & 42.4 & 27.9 & 61.3 & 57.0\\
DF   			& 65.0 & 58.7 & 45.8 & 32.0 & 67.0 & 67.1 \\
EF-LSTM   		& 66.3 & 65.0 & 44.1 & 43.6 & 67.0 & 64.3 \\
EF-SLSTM		& 72.5 & 70.9 & 40.7 & 41.2	& 56.6 & 51.4 \\
EF-BLSTM 		& 63.8 & 49.6 & 42.4 & 38.1 & 58.5 & 58.9 \\
EF-SBLSTM 		& 62.5 & 49.0 & 37.3 & 33.2 & 63.2 & 63.3 \\
MV-LSTM			& 72.5 & 72.3 & 45.8 & 43.3 & 57.6 & 48.2 \\
BC-LSTM    		& 70.0 & 70.1 & 45.0 & 45.1 & 72.6 & 72.9 \\ 
TFN      		& \textbf{72.5}	& \textbf{72.6} & 45.0 & 41.0 & 63.2 & 61.7 \\ 
MARN			& 71.3 & 70.2 & 48.3 & 44.9 & 81.1 & \textbf{81.2} \\ 
MFN				& 70.0 & 69.3 & 51.7 & 51.6 & \textbf{81.1} & 80.4 \\
\Xhline{0.5\arrayrulewidth}
MFN \ours       & 66.3 & 63.9 & \textbf{53.3} & \textbf{52.4} & 80.2 & 79.8 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Sentiment prediction results on ICT-MMMO, YouTube and MOUD test sets. The best results are highlighted in bold and $\Delta_{SOTA}$ shows the change in performance over previous state of the art. Improvements are highlighted in green. The \ours \ significantly outperforms the current state of the art across all evaluation metrics.}
\label{mmmo+you+moud}
\end{table}

==> tables/mosi.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\definecolor{gg}{RGB}{45,190,45}

\begin{table}[t!]
\fontsize{7.5}{10}\selectfont
%\centering
\setlength\tabcolsep{1.3pt}
\begin{tabular}{l : *{16}{K{1.09cm}}}
\Xhline{3\arrayrulewidth}
Dataset & \multicolumn{5}{c}{\textbf{CMU-MOSI}} \\
Task & \multicolumn{5}{c}{Sentiment} \\
Metric       & A$^{2}$ & F1 & A$^{7}$ & MAE & Corr\\ 
\Xhline{0.5\arrayrulewidth}
Majority       & 50.2 &   50.1   &	 17.5	&     1.864 &  0.057  \\
RF         & 56.4 &  56.3    &  21.3 	&		-     	&  - \\ 
SVM-MD     & 71.6 &   72.3   & 26.5  	& 1.100     &  0.559 \\ 
THMM		& 50.7	& 45.4	& 17.8& - & -\\
SAL-CNN    & 73.0 &   -      &  -	&  -        	& -\\ 
C-MKL          & 72.3 &   72.0   &  30.2	&  -       		& -\\
EF-HCRF	& 65.3& 65.4& 24.6& - & -\\
MV-HCRF	& 65.6& 65.7 & 24.6 & - & -\\
DF              & 72.3 &   72.1   &  26.8 	& 1.143     &  0.518 \\
MV-LSTM			& 73.9 &   74.0   &  33.2	& 1.019 &  0.601 \\
BC-LSTM         & 73.9 &   73.9   &  28.7	& 1.079 &  0.581 \\ 
\Xhline{0.5\arrayrulewidth}
EF     & 75.1 & 74.6 & \textbf{33.5} & 1.02 & 0.639 \\
EF \ours   & 75.2 & 75.3 & 32.8 & 1.02 & 0.629 \\
\Xhline{0.5\arrayrulewidth}
TF     & 75.1 & 75.1 & 27.0 & 1.10 & 0.643 \\
TF \ours   & 74.5 & 74.5 & 30.9 & 1.05 & 0.624 \\
\Xhline{0.5\arrayrulewidth}
MARN   & 74.8 & 74.8 & 30.6 & 1.05 & 0.617 \\
MARN \ours & 75.5 & 75.4 & 31.2 & 1.05 & 0.640 \\
\Xhline{0.5\arrayrulewidth}
MFN        & 76.1 & 76.0 & 28.7 & 1.04 & 0.634 \\
MFN \ours  & \textbf{78.1} & \textbf{78.1} & \textbf{36.2} & \textbf{0.963} & \textbf{0.662} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Sentiment prediction results on CMU-MOSI test set for comparing the performance of \ours \ with existing methods for multimodal fusion. The best results are highlighted in bold. \ours \ achieves better results as compared to their discriminative counterparts. A$^C$ = multiclass accuracy across $C$ classes, MAE = Mean Absolute Error, $r$ = Pearson's correlation.}
\label{mosi}
\end{table}
